$\alpha$-$\beta$-Factorization and the Binary Case of Simon's Congruence

In 1991 H\'ebrard introduced a factorization of words that turned out to be a powerful tool for the investigation of a word's scattered factors (also known as (scattered) subwords or subsequences). Based on this, first Karandikar and Schnoebelen introduced the notion of $k$-richness and later on Barker et al. the notion of $k$-universality. In 2022 Fleischmann et al. presented a generalization of the arch factorization by intersecting the arch factorization of a word and its reverse. While the authors merely used this factorization for the investigation of shortest absent scattered factors, in this work we investigate this new $\alpha$-$\beta$-factorization as such. We characterize the famous Simon congruence of $k$-universal words in terms of $1$-universal words. Moreover, we apply these results to binary words. In this special case, we obtain a full characterization of the classes and calculate the index of the congruence. Lastly, we start investigating the ternary case, present a full list of possibilities for $\alpha\beta\alpha$-factors, and characterize their congruence.

==> ideas.tex <==
\section{Ideas and Open Questions}
\todofpa{is $k>|w|$? otherwise check edge cases}
\todojho{In general no. In my master's thesis is classified the binary congruence classes which are infinite. Note that for example \(w = a^{k-2}ba^{b-2}\cdots ba^{k-2}\) for \(|w|_b < k\) is still a singleton class but much longer than \(k\)}
\subsection{\(\Sigma_3^* \mathord{/}{\sim_k}\)}

\begin{definition}
  Let \(w = \alpha_0\beta_1\cdots \beta_{\iota(w)}\alpha_{\iota(w)}\in\Sigma_2^*\) be a binary word and \(\ta\in\Sigma_2\).
  Define
  \[
    \iota(w, \ta) = \iota(w) + \delta_{\ta\in\alphabet(\alpha_{\iota(w)})}\cdot|\alpha_{\iota(w)}|, \qquad \m(w, \ta) = \m(w)\cdot
    \begin{cases}
      \alpha_{\iota(w)} & \ta \preceq \alpha_{\iota(w)}, \\
      \varepsilon      & \ta \npreceq \alpha_{\iota(w)},
    \end{cases}
  \]
  and \(\rev\iota(\ta, w)\) symmetric.
\end{definition}

\todo[inline]{this one is above}

\begin{lemma}\label{lemabaohnea}
Let $w,\tilde{w}\in\Sigma_{\geq 3}^{\ast}$ with $\iota(w)=\iota(\tilde{w})=1$ and $\alpha_0=\alpha_1=\varepsilon$.
Then $w\sim_k\tilde{w}$ for $k\geq 2$ iff $\w(\tilde{w})=\w(w)$, $m(\tilde{w})=m(w)$, $w[2..|w|-1]\sim_{k} \tilde{w}[2..|\tilde{w}|-1]$, and $\tilde{\alpha}_0=\tilde{\alpha}_1=\varepsilon$.
\end{lemma}

\begin{proof}
Let $w[1]=0$ and $w[|w|]=1$. Notice that both are unique in $w$, since $\iota(w)=1$. Choose $u\in(\Sigma\backslash\{0,1\})^{\ast}$ with $w=0u1$.

\medskip

Consider first $w\sim_k\tilde{w}$. If $m(\tilde{w})\neq 1$, then $1\in\inner(\ar_1(\tilde{w}))$, thus $1m(\tilde{w})\preceq \tilde{w}$ but $1m(\tilde{w})\not\preceq w$. Thus $\tilde{\beta}(|\tilde{\beta}|)=m(w)=1$. By symmetry we have $\tilde{\beta}[1]=0$.   If $\tilde{\alpha_0}\neq\varepsilon$, we would have $\tilde{w}[1]0\preceq\tilde{w}$ - again a contradiction.
By symmetry we have $\tilde{\alpha_1}=\varepsilon$. This implies $\tilde{\beta_1}=0\tilde{u}1$ with $\letters(\tilde{u})=\Sigma\backslash\{0,1\}$. It remains to show $u\sim_{k}\tilde{u}$. If there existed $v\in\Sigma^{k}$ with $v\preceq u$ and $v\not\preceq\tilde{u}$, then $0v1\preceq w$. On the other hand
by $\letters(u)=\Sigma\backslash\{0,1\}=\letters(\tilde{u})$, $0v1\not\preceq \tilde{w}$ a contradiction. The second inclusion follows by symmetry.

\medskip

The second direction is immediate.\qed
\end{proof}

Lemma~\ref{lemabaohnea} implies for $\Sigma_3$ the following restriction.

\begin{corollary}
Let $w,\tilde{w}\in\Sigma_3^{\ast}$ with $\iota(w)=\iota(\tilde{w})=1$ and $w\sim_k\tilde{w}$ for $k\geq 2$
and $\alpha_0=\alpha_1=\varepsilon$, i.e., w.l.o.g. $\beta_1=01^{\ell}2$. Then $\tilde{w}=01^{\tilde{\ell}}2$
with $1^{\ell}\sim_k 1^{\tilde{\ell}}$ for some $\ell,\tilde{\ell}\in\N$.
\end{corollary}

\begin{lemma}
Let $w,\tilde{w}\in\Sigma_{\geq 3}^{\ast}$ with $\iota(w)=\iota(\tilde{w})=1$, $\alpha_0=\varepsilon$, $\alpha_1\neq \varepsilon$. 
Then we have $w\sim_k\tilde{w}$ for $k\geq 2$ iff $m(w)=m(\tilde{w})$, $\w(w)=\w(\tilde{w})$, $\tilde{\alpha}_0=\varepsilon$ and $u\alpha_1\sim_k \tilde{u}\tilde{\alpha}_1$ for $\beta_1=\w(w)u m(w)$ and $\tilde{\beta}=\w (w)\tilde{u}m(w)$.
\end{lemma}

\begin{proof}
Consider first $w\sim_k \tilde{w}$.
Let $\beta=0u1$. Notice $0,1\not\in\letters(u)$ and $1\not\in\letters(\alpha_1)$. By $\alpha_1\neq\varepsilon$, there exists $y\in\letters(\alpha_1)$ and $y\neq 0$. If $\tilde{\beta}[1]=x\neq 0$
then $x0\preceq\tilde{w}$ but $x0\not\preceq w$ - a contradiction. With the same argument $\tilde{\alpha_0}=\varepsilon$.\\
\textbf{Suppose}: $m(\tilde{w})=x\neq 1$\\
Since $x\in\letters(\beta)$, we have $x1y\preceq w$. This implies $1y\in\letters(\tilde{\alpha}_1)$.
Thus, $1x1y\preceq\tilde{w}$ which implies $x1y\in\letters(\alpha_1)$. Thus $(x1)^2y\preceq w$. Inductively,
we get $(x1)^{\omega}y\in\letters(\alpha_1)$ - a contradiction.\\
Thus there exists $\tilde{u}\in(\Sigma\backslash\{0,1\})^{\ast}$ with $\tilde{\beta}=0\tilde{u}1$. Let $v\preceq u\alpha_1$ with $v\in\Sigma^k$. Thus there exists $v_1,v_2$ with $v_1\preceq u$ and $v_2\preceq\alpha_1$. This implies $v\preceq w$ and thus, $v\preceq \tilde{w}$. Since $v\preceq u\alpha_1$, we have $0\not\in\letters(v)$ and thus $v\preceq 0^{-1}\tilde{w}$. Since we are done if $v\preceq \tilde{u}\tilde{\alpha}_1$, assume $v=\tilde{v}_11\tilde{v}_2$ with
$\tilde{v}_1\preceq\tilde{u}$, $\tilde{v}_2\preceq\tilde{\alpha}_1$ but $1\tilde{v}_2\not\preceq\tilde{\alpha}_1$ (this factorization is well defined by $m(w)=1$). Because $v\preceq u\alpha_1$ and $1\not\in\letters(u)$, we obtain $1\in\letters(\alpha_1)$. This leads to $1\in\letters(\tilde{\alpha}_1)$ since $11\preceq w\sim_k\tilde{w}$ and $1\not\in\letters(\tilde{u})$. Choose $z_1,z_2\in\letters(\tilde{\alpha}_1)^{\ast}$ with $\tilde{\alpha}_1=z_11z_2$ and $1\not\in\letters(z_1)$. Thus, we have $\tilde{v}_2\not\preceq z_2$. Note that we have $\tilde{v}_11\tilde{v}_2=v_1v_2$ and by $1\not\in\letters(v_1)$ we have $1\tilde{v}_2\preceq v_2$. This implies $11\tilde{v_2}\preceq w\sim_k\tilde{w}$ and again by $m(\tilde{w})=1$ and the choice of $z_2$ we have $\tilde{v}_2\preceq z_2$ - a contradiction. Thus, we have $u\alpha_1\sim_k\tilde{u}\tilde{\alpha}_1$. The second inclusion follows by symmetry.
\medskip

The second direction is immediate.\qed
\end{proof}

Similarly, we can obtain the following results for $\Sigma_3$.

\begin{corollary}
Let $w,\tilde{w}\in\Sigma_3^{\ast}$ with $\iota(w)=\iota(\tilde{w})=1$ and $w\sim_k\tilde{w}$ for $k\geq 2$
and $\alpha_0=\varepsilon$ and $\alpha_1\neq \varepsilon$. , i.e., w.l.o.g. $\beta_1=01^{\ell}2$. Then there exist $\ell,\tilde{\ell}\in\N$ with $\tilde{w}=01^{\tilde{\ell}}2$, $\letters(\alpha_1),\letters(\tilde{\alpha_1})\subseteq\{1,2\}^{\ast}$ and $w\sim_k\tilde{w}$ iff $1^{\ell}\alpha_1\sim_k1^{\tilde{\ell}}\tilde{\alpha}_1$.
\end{corollary}

\begin{lemma}
Let $w,\tilde{w}\in\Sigma_{\geq 3}^{\ast}$ with $\iota(w)=\iota(\tilde{w})=1$, $\alpha_0, \alpha_1\neq \varepsilon$. 
Then we have $w\sim_k\tilde{w}$ for some $k\geq 2$?
\end{lemma}

\begin{proof}
Let $w\sim_k\tilde{w}$ and $\beta_1=0u1$. By the definition of arches, we have $1\not\in\letters(\alpha_0)$ and
$0\not\in\letters(\alpha_1)$, thus $10\not\preceq w$. If $1\not\in\tilde{\beta}_1$, we have $1\in\tilde{\alpha}_0,\tilde{\alpha}_1$. By $w\sim_k\tilde{w}$ the $0$ occurs only before the $1$ and thus $0\not\in\tilde{\beta}_1$. Thus, $0\in\tilde{\alpha}_1$ and $10\preceq\tilde{w}$ - a contradiction. By symmetry, we get $0,1\in\letters(\tilde{\beta}_1)$.  
\todo[inline]{TBC}
\end{proof}

\newpage
\begin{lemma}[Ternary \(\beta\) classification]
Let $w,\tilde{w}\in\Sigma_3^{\ast}$ with $\iota(w)=\iota(\tilde{w})=1$ and $w\sim_k\tilde{w}$.
\begin{itemize}
\item If $|\letters(\alpha_0)|=0$ then $\beta=01^{\ell}2$ (up to a permutation of $\Sigma$). If moreover $|\letters(\alpha_1)|=0$ then
    \begin{itemize}
    \item if $\ell\leq k-1$, then $w=\tilde{w}$,
    \item if $\ell\geq k$, then $\tilde{w}=01^{\tilde{\ell}}2$ for some $\tilde{\ell}\geq k$.
    \end{itemize}
    or if $|\letters(\alpha_1)|=1$ then  
    \begin{itemize}
    \item if $\ell\leq k-1$ or $|\alpha_i|\leq k-2$, then $w=\tilde{w}$,
    \item if $\ell\geq k$ and $|\alpha_i|\geq k-1$, then $\tilde{w}=01^{\tilde{\ell}}2^r$ if $\m(w)=\letters(\alpha_1)$ or $\tilde{w}=01^{\tilde{\ell}}21^r$ if $\m(w)\neq\letters(\alpha_1)$ for some $\tilde{\ell},r\geq k$.
    \end{itemize}
    or if $|\letters(\alpha_1)|=2$ then  
    \begin{itemize}
    \item 
    \end{itemize}
\end{itemize}
old
\begin{itemize}
\item If $|\letters(\alpha_0)|=|\letters(\alpha_1)|=2$ then $w=\tilde{w}$.
\todo[inline]{TBC}
\end{itemize}
  
\end{lemma}
\begin{proof}
  Consider first \(|\alphabet(\alpha_0)|=0\). Thus, $\letters(\beta)=\Sigma_3$. Let $\m(w)=2=\beta(|\beta|)$ and $\w(w)=0=\beta[1]$.
  By the definition of arches we have w.l.o.g. $\beta=01^{\ell}2$. By $w\sim_2\tilde{w}$, we obtain $\tilde{\beta}=01^{\tilde{\ell}}2$ for some
  $\tilde{\ell}\in\N$. Now we distinguish cases based on $\letters(\alpha_1)$.\\
  \textbf{case 1:} $\letters(\alpha_1) = \emptyset$:\\
  If $\ell\leq k-1$, $1^k\not\preceq w$. Thus, $\tilde{\ell}\leq k-1$. If $\ell<\tilde{\ell}$ we would get $1^{\tilde{\ell}}\preceq \tilde{w}$ but $1^{\tilde{\ell}}\not\preceq w$. Hence, $w=\tilde{w}$. On the other hand, if $\ell\geq k$, we have $[w]_{\sim_k}=\{01^{\tilde{\ell}}2|\,\tilde{\ell}\geq k\}$ we have since we only consider $\sim_k$.\\
  \textbf{case 2:} $\letters(\alpha_1) = \{1\}$ of $\letters(\alpha_1) = \{2\}$\\
  Thus, $w = \beta 1^{s_1}$ or $w = \beta 2^{s_2}$ for some $s_1,s_2 \in \mathbb{N}$. 
  
  \medskip
  

 
  
  
  \begin{description}
    \item[\(|\alphabet(\alpha_0)| = |\alphabet(\alpha_1)| = 2\)] Because \(\alpha_0\beta = \ar_1(w)\) and \(\beta\alpha_1 = \ra_1(w)\), the last and first letter of \(\beta\) are the unique missing letter from \(\alphabet(\alpha_0)\) and \(\alphabet(\alpha_1)\) respectively.
      If \(\alphabet(\alpha_0) = \alphabet(\alpha_1)\) we thus conclude \(|\beta| = 1\).
      Therefore, assume without loss of generality \(\alphabet(\alpha_0) = \{0,1\}\) and \(\alphabet(\alpha_1) = \{1,2\}\) and thus \(\beta = 01^\ell2\) for some \(\ell\in\mathbb N_0\).

      Consider \(\ell,\ell'\in [k - \iota(\alpha_0, 1) - \iota(\alpha_1,1)]_0\).
      We show that \(\alpha_001^\ell2\alpha_1 \sim_k \alpha_001^{\ell'}2\alpha_1\) implies \(\ell = \ell'\).
      Suppose \(\ell < \ell'\), then for \(v = \m(\alpha_0,1) \cdot 1^{\ell'} \cdot \w(1,\alpha_1)\) we have \(v \preceq \alpha_001^{\ell'}2\alpha_1\) but \(v\npreceq \alpha_001^{\ell}2\alpha_1\), a contradiction.

      \todo[inline]{Show that all larger \(\ell\) are equivalent to a smaller one.}
    \item[\(|\alphabet(\alpha_0)| \neq |\alphabet(\alpha_1)| = 2\)]
    \item[]
      
  \end{description}
\end{proof}
  
% \subsection{Transposing the Problem, \(\Sigma_n^* \mathord{/}{\sim_2}\)}
% 
% For \(n \leq 2\) we have already solved the problem.
% We can divide words based their alphabets.
% Let \(w\in \Sigma_n\).
% If \(\alphabet(w) \subset \Sigma_n\), then we already classified it by induction.
% If \(\alphabet(w) = \Sigma_n\), then we know \(\iota(w) \geq 1\).
% There exists only a single class of words \(w\) with \(\iota(w) \geq 2\).
% Therefore, assume \(\iota(w) = 1\) and thus \(w = \ar_1(w)\cdot \alpha_0 = \alpha_1 \cdot \ra_1(w)\).
% 
% \(\alpha_0\) and \(\alpha_1\) are fixed up to \(\sim_1\) equivalence and therefore are in bijective correspondence with \(\prod_{i \in [n-1]_0} \binom{\Sigma}{i}\).
% Denote by \(\sigma_1,\rev{\sigma}_1 \in \mathcal S_n\) the bijection on the alphabet \(\Sigma_m\), given by the modi sequence of the (nested) arches \(\ar_1(w)\) and \(\ra_1(w)\) respectively.
% \todo[inline]{Consider whether the inner arches and reverse arches overlap}

% 

\subsection{Imported Proofs}

\todojho{By \Cref{prop:simon-equiv-iff-equiv-with-same-alpha} we can assume that \(\alpha_i = \tilde\alpha_i\) by adding equivalence as an assumption (which is not a real restriction)}

\begin{lemma}
  Let \(w,\tilde w\in\Sigma^*\) with \(1 = \iota(w) = \iota(\tilde w)\) and \(\letters(\alpha_0) = \letters(\alpha_1) \in \binom{\Sigma}{|\Sigma|-1}\).
  We have \(w \sim_k \tilde w\), if and only if, \(\alpha_i \sim_{k-1} \tilde\alpha_i\) for all \(i\in[1]_0\).
\end{lemma}
\begin{proof}
  In both directions, we have \(\beta = \tilde\beta \in \Sigma\) by uniqueness of their first and last letter.
  The claim then follows from \Cref{prop:beta-equal-implies-equiv-iff-alpha-equiv}.\qed
\end{proof}

\begin{lemma}
  Let \(w,\tilde w\in\Sigma_3^*\) with \(1 = \iota(w) = \iota(\tilde w)\) and \(|\letters(\alpha_0)| = |\letters(\alpha_1)| = 2\) and \(|\letters(\alpha_0) \cap \letters(\alpha_2)| = 1\).
  Therefore, \(\beta = \tx\ty^\ell\tz\) and \(\tilde\beta = \tx\ty^{\tilde\ell}\tz\) with \(\tx,\ty,\tz \in\Sigma_3\) pairwise different.
  We have \(w \sim_k \tilde w\), if and only if, \(\alpha_i \sim_{k-1} \tilde\alpha_i\) for all \(i\in[1]_0\) and \(\min(k - c, \ell) = \min(k - c,\tilde\ell)\), where \(c \coloneqq \iota(\alpha_0) + \delta_{\ty\in \re(\alpha_0)} + \iota(\alpha_1) + \delta_{\ty \in\er(\alpha_1)}\).
\end{lemma}
\begin{proof}

  \qed
\end{proof}

\begin{lemma}
  Let \(w,\tilde w\in\Sigma_3^*\) with \(1 = \iota(w) = \iota(\tilde w)\) and \(|\letters(\alpha_0)| = |\letters(\alpha_1)| = 2\) and \(|\letters(\alpha_0) \cap \letters(\alpha_2)| = 1\).
  Therefore, \(\beta = \tx_1\ty_1^\ell\tz_1\) and \(\tilde\beta = \tx_2\ty_2^{\tilde\ell}\tz_2\) with \(\tx_i,\ty_i,\tz_i \in\Sigma_3\) pairwise different for \(i\in[1]_0\) and \(\ell,\tilde \ell\in\mathbb N\).
  We have \(w \sim_k \tilde w\), if and only if, \(k = 1\) or \(k \geq 2\), \(\tx_1\ty_1\tz_1 = \tx_2\ty_2\tz_2\) and \(\min(k,\ell) = \min(k,\tilde \ell)\).
\end{lemma}
\begin{proof}

  \qed
\end{proof}


\todojho{From Master's thesis; if usefull recheck proof!}
In this last lemma, we show another decomposition, this time of \(1\)-universal words with non-trivial \(\alpha_i\).
In the lemma and proof we consider factorizations of \(\alpha_i\).
We regard \(\alpha_0\) and \(\alpha_1\) as words over the alphabets \(\Sigma\setminus\{\m_1(w)\}\) and \(\Sigma\setminus\{\w_1(w)\}\) respectively.
Furthermore, for simplicity, we assume that the \(\alpha_i\) do not have more than \(k-1\) arches, as we can always exchange \(\alpha_i\) with more than \(k-1\) arches by \Cref{prop:beta-equal-implies-equiv-iff-alpha-equiv}.
\begin{lemma}
  Let \(w, \tilde w \in \Sigma^*\) such that \(1 = \iota(w) = \iota(\tilde w)\) and \(\iota(\alpha_i), \iota(\tilde\alpha_i) \leq k - 1\) for \(i\in[1]_0\).
  Then \(w \sim_k \tilde w\), if and only if,
  \begin{itemize}
    \item \(\alpha_i \sim_{k-1} \tilde\alpha_i\) for all \(i\in[1]_0\),
    \item \(\re(\alpha_0) \cdot \beta_1(u) \cdot \re(\alpha_1) \sim_{\max(0, k - \ell_0 - \ell_1)} \re(\tilde\alpha_0) \cdot \tilde\beta_1 \cdot \re(\tilde\alpha_1)\) where \(\ell_i \coloneqq \iota(\alpha_i) = \iota(\tilde\alpha_i)\) for all \(i\in[1]_0\).
  \end{itemize}
\end{lemma}
\begin{proof}
  \todojho{\(\implies\) follows by exchanging \(\alpha\)}

  Assume \(\ell_0,\ell_1 \geq 1\), then either \(\beta = \tilde\beta \in\Sigma\) or there exist \(\tx,\ty\in\Sigma\) such that \(\beta = \tx\beta_i\ty\) and \(\tilde\beta = \tx\tilde\beta_i\ty\).

  \begin{align*}
    w &=
    \ar_{1..\ell_0}(\alpha_0)\cdot\re(\alpha_0) \cdot \tx\beta_i\ty\cdot \er(\alpha_1) \cdot \ra_{1..\ell_1}(\alpha_1) \\
    &\sim_k \ar_{1..\ell_0}(\alpha_0)\cdot\re(\tilde\alpha_0) \cdot \tx\tilde\beta_i\ty\cdot \er(\tilde\alpha_1) \cdot \ra_{1..\ell_1}(\alpha_1) \tag{} \\
    &\sim_k \ar_{1..\ell_0}(\tilde\alpha_0)\cdot\re(\tilde\alpha_0) \cdot \tx\tilde\beta_i\ty\cdot \er(\tilde\alpha_1) \cdot \ra_{1..\ell_1}(\tilde\alpha_1) \tag{\Cref{prop:beta-equal-implies-equiv-iff-alpha-equiv}} \\ 
    &\sim_k \tilde w.
  \end{align*}

  \begin{align*}
    \re(\alpha_0) \cdot \beta \cdot \er(\alpha_1)
    &\sim_{k-\ell_0-\ell_1}  \re(\tilde \alpha_0) \cdot \tilde \beta \cdot \er(\tilde\alpha_1) \\
    &\sim_{k-1-\ell_1} \re(\alpha_0) \cdot \tilde \beta \cdot \er(\tilde \alpha_1) \\
    &\sim_{k-\ell_0-1} \re(\alpha_0) \cdot \tilde \beta \cdot \er(\alpha_1) \\
  \end{align*}
  \qed
\end{proof}

==> tikzlibrarywords.code.tex <==
% Really hacky implementation of basic word diagrams.
% The main idea is to curve words and to add tick marks via a decoration, that is, to rewrite how the path is drawn.
% The advantage of this approach is that "what it means to be a word" can be encapsulated into a style.
% Therefore, you do not have to add extra noddes to curve words.
% Furthermore, compared to line caps, the endpoints are at the actual desired positions so words match up.
% Since words are normals paths you can use TikZ commands such as \for to draw multiple words at once.
% A disadvantage is that this implementation is not realy robust, therefore, applying more fancy extra decorations to words may not work as desired. 

% EXAMPLE:
%    \foreach \x [remember=\x as \lastx, count=\i] in {2,5,7}{
%      \ifnum\lastx=0
%        \draw[point] (\lastx, 2.5) -- ++(0, -.475);
%      \fi
%
%      \draw[word] (\lastx, 2) -- ++(\x-\lastx, 0);
%      \draw[uword] (\lastx, 2.5) -- ++(\x-\lastx, 0) node {\(\mathrm{ar}_{\i}(w)\)};
%      \draw[point] (\x, 2.5) -- ++(0, -.475);
%    }

% TODO
%
% - make dashes for points easier to draw "nicely"

\usepgfmodule{decorations}

\pgfdeclaredecoration{top word}{initial}
{
	\state{initial}[width=\pgfdecoratedpathlength]{
		\pgfpathlineto{\pgfpoint{0}{0.15cm}}
		\pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{0.15cm}}
		\pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{0cm}}
	}
}

\pgfdeclaredecoration{bot word}{initial}
{
	\state{initial}[width=\pgfdecoratedpathlength]{
		\pgfpathlineto{\pgfpoint{0}{-0.15cm}}
		\pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{-0.15cm}}
		\pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{0cm}}
	}
}

\pgfdeclaredecoration{center word}{initial}
{
	\state{initial}[width=\pgfdecoratedpathlength]{
		\pgfpathlineto{\pgfpoint{0}{-0.075cm}}
		\pgfpathmoveto{\pgfpoint{0}{0.0cm}}
		\pgfpathlineto{\pgfpoint{0}{0.075cm}}
		\pgfpathmoveto{\pgfpoint{0}{0.0cm}}
		\pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{0}}
		\pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{-0.075cm}}
		\pgfpathmoveto{\pgfpoint{\pgfdecoratedpathlength}{0.0cm}}
		\pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{0.075cm}}
		\pgfpathmoveto{\pgfpoint{\pgfdecoratedpathlength}{0.0cm}}
	}
}

\tikzset{
	uword/.style={
			rounded corners, thick, decorate, decoration={top word}, line cap=round, every node/.style = {yshift=1.15mm, above, midway}
		},
	dword/.style={
			rounded corners, thick, decorate, decoration={bot word}, line cap=round, every node/.style = {yshift=-1.15mm, below, midway}
		},
	word/.style={
			thick, decorate, decoration={center word}, line cap=round, every node/.style = {above, midway}
		},
	point/.style={
			thick, dash pattern=on 1pt off 2pt, rounded corners, line cap=round%, dash expand off
		},
        brace/.style={
                        decorate, decoration = {brace,amplitude=0.2cm},thick, line cap=round, every node/.style = {above, midway, inner sep=0.25cm, allow upside down}
                },
        innerLabel/.style={
                        anchor=center,fill=white,inner sep=0.5pt
                },
        innerLabelStart/.style={
                        innerLabel, pos=0, right
                },
        outerLabelStart/.style={
                        pos=0, left
                },
        innerLabelEnd/.style={
                        innerLabel, pos=1, left
                }
}

\newcommand{\point}[2][]%
{\draw[thick, -{Stealth[round]}, line cap=round] ($ ({#2}) + (0, 0.3) $) node[above] {\({#1}\)} -- ++(0, -0.3)}

\newcommand{\upoint}[2][]%
{\draw[thick, -{Stealth[round]}, line cap=round] ($ ({#2}) + (0, -0.3) $) node[below] {\({#1}\)} -- ++(0, 0.3)}

